Alexandria: Extensible Framework for Rapid Exploration of Social Media

The Alexandria system under development at IBM Research provides an extensible framework and platform for supporting a variety of big-data analytics and visualizations. The system is currently focused on enabling rapid exploration of text-based social media data. The system provides tools to help with constructing "domain models" (i.e., families of keywords and extractors to enable focus on tweets and other social media documents relevant to a project), to rapidly extract and segment the relevant social media and its authors, to apply further analytics (such as finding trends and anomalous terms), and visualizing the results. The system architecture is centered around a variety of REST-based service APIs to enable flexible orchestration of the system capabilities; these are especially useful to support knowledge-worker driven iterative exploration of social phenomena. The architecture also enables rapid integration of Alexandria capabilities with other social media analytics system, as has been demonstrated through an integration with IBM Research's SystemG. This paper describes a prototypical usage scenario for Alexandria, along with the architecture and key underlying analytics.

==> 08-many-users.tex <==

\section{Scaling to Many Users}

\rick{??}


==> 09-experiments.tex <==


\section{Benchmarking and Experiments}
\label{sec:experiments}

This section presents some highlights from
executions of the Alexandria system,
including both actual runs and controlled benchmarking.

\subsection{Tweet processing}

The current system is focused on a fixed set of English-language
Tweets from the Twitter Decahose (10\% of all Tweets).
With regards to background ingestion and initial processing,



Figure \ref{fig:tweet-ingestion-times} gives high-level information about
the time it takes to ingest and index tweets.  
The current Alexandria infrastructure uses a 4 node cluster,
with 1 as master and 3 as slaves; each node has
64MB of memory.
As shown in the table, the parallelism afforded by the 4 nodes
gives a substantial increase.
The table shows the time needed to ingest and index one day's worth
of the English-language tweets from the Twitter Decahose
(about 400 million tweets), to build an index 
(with size about 128 GB).
While the use of 80 mapper services reduces the time needed
to about 2 hours per day, using 17K mappers (the maximum available)
reduces the time to about 1 hour.  
It remains open to determine the smallest number of mappers that
achieves this 1 hour performance time.

\rick{The numbers in Figure \ref{fig:tweet-extraction-times}
seem odd, because it is not linear.  Was there some background
process running for the 1M tweet run??? We will need to
re-run these tests, I think}

As described in Section \ref{sec:arch}, a key processing step in the
exploration processing is to perform an extraction and annotation
step once a targeted set of tweets and authors has been
identified by a Domain Model.
Figure \ref{fig:tweet-extraction-times}
shows the time needed for this step, for two representative
sets of tweets, one with about 0.5 million tweets and the other
with about 1 million.
In the current system there are four parts to the extraction
processing step.
First, SOLR is used to create an index in main memory specific
to the targeted tweets.
Second, the actual tweet data is pulled into SOLR.
Third, the tweet data is pulled over the wire into
the extraction service component.
Finally, this service annotates the tweet and author information,
and writes them over the wire into three databases
(two couchDB and one SOLR). 
Looking forward, we expect to move towards an architecture 
with a single indexed data store, so that
we can perform the annotations ``in-place''.

\subsection{Term Generation and Clustering}

something here about variations on how term gen and clustering are done,
and measuring a notion of ``cluster stability''

\subsection{Direct Concept Generation}

something here about using term gen to get some inspiration words,
then selecting several disparate words, and then 
using word2vec to get concepts/clusters relating to each of those words

idea of varying different things
\begin{itemize}
\item background corpus (tweets vs articles vs ??)
\item number of background documents examined (e.g., 100, 500, 1K, 2K)
\item set of seed terms used (vaccination crisis, mandatory vaccinations, no-vaccination movement, anti-vaccination, $<<$ some diseases $>>$
\item number of terms generated
\item ???
\end{itemize}

How to measure quality
\begin{itemize}
\item Human inspection
\item cluster ``stability''
\item use Wikipedia listing of diseases where vaccination can treat as
a gold standard of some sort
\end{itemize}


